Grading Structure for Derivations of Group Algebras

In this paper we give a way of equipping the derivation algebra of a group algebra with the structure of a graded algebra. The derived group is used as the grading group. For the proof, the identification of the derivation with the characters of the adjoint action groupoid is used. These results also allow us to obtain the analogous structure of a graded algebra for outer derivations. A non-trivial graduation is obtained for all groups that are not perfect.

==> sections/CommChar.tex <==
The decomposed structure of $\Gamma$ stated by \label{decomp} does not give grading directly, but holds \Bcr{commchar}. \Bcr{commchar} is the first step to grading the $\Der$ algebra. \Bcr{commchar} will be used to show that $\Der$ is graded in \Bcr{sect:grading}.

\newcommand{\commsupp}[2]{\subgrdgen{[#1] \ostar [#2]}}
\newcommand{\commsuppab}{\commsupp{a}{b}}
\newcommand{\commsuppRHS}[4]{\CCup_{#1 \in [#3]} \CCup_{#2 \in [#4]} \subgrd{#1 #2}}
\newcommand{\commsuppRHSuvab}{\commsuppRHS{u}{v}{a}{b}}


\Bcr{commchar} motivates the following symbol

\begin{EqLNum}\label{commsuppdef}
     \commsuppab = \commsuppRHSuvab
\end{EqLNum}

\newcommand{\cla}{[a]}
\newcommand{\clb}{[b]}
\newcommand{\sga}{\subgrd a}
\newcommand{\sgb}{\subgrd b}
\newcommand{\homa}{\Hom(\sga)}
\newcommand{\homb}{\Hom(\sgb)}

\begin{lm}[Commutator's character]\label{commchar}
    \letthen{
        \item $a, b \in G$, 
        \item $\alpha$ is such a character that $\supp \alpha \le \subgrd a$, \todo{D subset?}
        \item $\beta$ is such a character that $\supp \beta \le \subgrd b$.
    }{
        \item $\supp \chcmm{\alpha}{\beta} \le \commsuppab$.
    }
\end{lm}
\begin{proof}
     \gnewcommand{\commchartemplateR}[5]{\Sum_{#5 \in G} #1(#3, #5) #2(#5, #4) - #2(#3, #5) #1(#5, #4)}
    \gnewcommand{\commchartemplate}[5]{\{#1, #2\}(#3, #4) = \commchartemplateR{#1}{#2}{#3}{#4}{#5}}
    \gnewcommand{\commchar}{\commchartemplate{\alpha}{\beta}{h}{g}{k}}
    %\renewcommand{\commchar}{\commchartemplate{\alpha}{\beta}{h}{x}{g}}

    \Bcr{mtrx} implies
    \begin{EqLN}
        \commchar
    \end{EqLN}
    Consider an arrow $(h, g)$ such that $\chcmm{\alpha}{\beta}(h, g) \neq 0$. Thus, there exists such $k \in G$
    \begin{EqLN}
        \begin{sqcases}
            \alpha(h, k)\beta(k, g) \neq 0 \\
            \beta(h, k)\alpha(k, g) \neq 0
        \end{sqcases}
    \end{EqLN}\todo{D sqcases?}
Therefore
    \begin{EqLNum}\label{commchar:eq:1}
        \begin{sqcases}
            \alpha(h, k) \neq 0 \wedge \beta(k, g) \neq 0 \\
            \beta(h, k) \neq 0 \wedge \alpha(k, g) \neq 0
        \end{sqcases}
    \end{EqLNum}
    
    Expressing \cref{commchar:eq:1} in terms of $\supp$
    
    \begin{EqLNum}\label{commchar:eq:2}
            \begin{sqcases}
            
            \begin{dcases}
                (h, k) \in \supp \alpha \subset \homa \\
                (k, g) \in \supp \beta \subset \homb
            \end{dcases} \\ \\
            \begin{dcases}
                (k, g) \in \supp \alpha \subset \homa \\
                (h, k) \in \supp \beta \subset \homb
            \end{dcases}
            \end{sqcases}
    \end{EqLNum}

    By \Bcr{maindef:lm:1}, an arrow $\phi$ belongs to a $\subgrd x$ iff its target $\trgt \phi$ belongs to $\subgrd x$. Thus, \cref{commchar:eq:2} implies
    
    \begin{EqLNum}\label{commchar:eq:3}
            \begin{sqcases}
               \begin{dcases}
                    h k\inv = u \in \cla \\
                    k g\inv = v \in \clb
                \end{dcases}\\ \\
                \begin{dcases}
                    k g\inv = u \in \cla \\
                    h k\inv = v \in \clb
                \end{dcases} 
            \end{sqcases}
    \end{EqLNum}

    Multiplying the equations within each curly brace \todo{D} in \cref{commchar:eq:3}\todo{"С чего бы?"}

    \newcommand{\uvdef}{,\textbf{ for } u \in \cla, v \in \clb}
    
    \begin{EqLN}
        \begin{sqcases}
           h g\inv = uv \\
           h g\inv = vu
        \end{sqcases}
        \uvdef
    \end{EqLN}

    By definition,\todo{W} $\trgt{h, g} = hg\inv$. By \Bcr{maindef:lm:1}

    \begin{EqLN}
        \begin{sqcases}
            (h, g) \in \Hom(\subgrd {uv}) \\
            (h, g) \in \Hom(\subgrd {vu})
        \end{sqcases}
    \end{EqLN}

    Since $[uv] = [u \cdot vu \cdot u\inv] = [vu]$

    \begin{EqLN}
        (h, g) \in \Hom(\subgrd {uv}) \uvdef
    \end{EqLN}

    By definition of $\commsuppab$ (see \cref{commsuppdef})

    \begin{EqLN}
        (h, g) \in \commsuppab
    \end{EqLN}

    Thus, $\chcmm{\alpha}{\beta}(h, g) \neq 0 \Rightarrow (h,g) \in \commsuppab$, therefore $\supp \chcmm{\alpha}{\beta} \subset \commsuppab$.

    \todo{examples}
\end{proof}



==> sections/Examples/Super.tex <==
Algebras, graded with $\ints_2$, are often referred to as \textbf{superalgebras}.

\begin{definition}
    \letthen{
        \item $H \le G$ --- $H$ be a subgroup in $G$,
    }
    {
        \item \textbf{$\bm H$ has an index 2 in $\bm G$} if there exists such $l \in G$ that:
        \begin{EqLN}
            G = H \sqcup lH
        \end{EqLN}
    }
\end{definition}

\begin{lm}
    \letthen{
        \item $H$ be a subgroup of index 2 in $G$,
    }
    {
        \item There exists such $r \in G$ that:
        \begin{EqLN}
            G = H \sqcup Hr
        \end{EqLN}
    }
\end{lm}
\begin{proof}
    \todo{TODO}
\end{proof}

\begin{corollary}
    \letthen{
        \item $H$ be a subgroup of index 2 in $G$.
    }
    {
        \item $H$ is normal in $G$,
        \item and $G/H \simeq \ints_2$.
    }
\end{corollary}
\begin{proof}
    \todo{TODO}
\end{proof}

\begin{lm}
    \letthen{
        \item $H \triangleleft G$ --- $H$ be a normal subgroup in $G$.
    }
    {
        \item $G/H$ is abelian $\iff G' \le H$. 
    }
\end{lm}
\begin{proof}
    \todo{TODO}
\end{proof}

\begin{corollary}\label{ex:cl:1}
    \letthen{
        \item $H$ be a subgroup of index 2 in $G$.
    }
    {
        \item \begin{EqLN}
            G' \le H
        \end{EqLN}
    }
\end{corollary}
\begin{proof}
    \todo{TODO}
\end{proof}

\begin{example}
    \letthen{
        \item There exists a subgroup $H$ of index 2 in $G$.
    }
    {
        \item There exist such $\Der_0, \Der_1 \subset \Der$ that:
        \begin{EqLN}\label{ex:eq:1}
            \Der = \Der_0 \oplus \Der_1 \\
        \end{EqLN}
        And \cref{ex:eq:1} is a grading of $\Der$.
    }
\end{example}
\begin{proof}
    By \Bcr{ex:cl:1}:
    \begin{EqLN}
        G/H \simeq \ints_2
    \end{EqLN}
\end{proof}

==> sections/GradingOtherQ.tex <==

\begin{st}\label{grad:st:1}\todo{R}
    \letthen{
        \item $N \triangleleft G$ be a normal subgroup in $G$,
        \item $G' \subset N$.
    }{
        \item $G/N$ is an abelian group.
    }
\end{st} 

%\begin{lm}\label{normadjplus}
%    \letthen{
%        \item $N, M \triangleleft G$ be normal subgroups in $G$,
%        \item $N \subset M$.
%    }
%    {
%        \item for any $a \in G$ there exists a set $U \subset G$
%        \begin{EqLN}
%            aM = \SqCup_{u \in U} uN
%        \end{EqLN}
%    }
%\end{lm}
%\begin{proof}
%    \begin{enumerate}
%        \item\label{grading:item:1} First, we prove \Bcr{normadjplus} for the case of $a = e$.
%
%        Consider $u \in G$. Then
%        \begin{EqLN}\label{grading:eq:1}
%            uN \cap M \neq \O \iff u \in M
%        \end{EqLN}
%        \begin{subproof}[Proof for \cref{grading:eq:1}]
%            $(\Leftarrow)$ is obvious. For $u \in M$
%            \begin{EqLN}
%                uN \subset M
%            \end{EqLN}
%
%            $(\Rightarrow)$ Consider such $u \in G$ that
%            \begin{EqLN}
%                M \cap uN \neq \O
%            \end{EqLN}
%
%            Therefore, there exist $m \in M, n \in N$
%            \begin{EqLN}
%                m = un 
%            \end{EqLN}
%
%            Since $N \subset M$
%            \begin{EqLN}
%                u = mn\inv \in M 
%            \end{EqLN}
%        \end{subproof}
%
%        By \cref{grading:eq:1}
%        \begin{EqLN}
%            M = \CCup_{u \in M} uN
%        \end{EqLN}
%
 %       Therefore, there exists\todo{Elaborate} such a set $U_0 \subset M$ that
%        \begin{EqLN}
%            M = \SqCup_{u \in U_0} uN
%        \end{EqLN}
%
%        \item Consider an arbitrary $a \in G$. By \cref{grading:item:1}
%        \begin{EqLN}
%            aM = a\Bigg(\SqCup_{u \in U_0} uN \Bigg) = \SqCup_{u \in U_0} auN = \SqCup_{u \in U_0} auN = \SqCup_{v \in aU_0} vN
%        \end{EqLN}
%    \end{enumerate}
%\end{proof}

\begin{thm}[Generalization of \Bcr{grad}]
    \letthen{
        \item $N \triangleleft G$ be a normal subgroup in $G$,
        \item $G' \subset N$.
    }
    {
        \item$\Der$ is graded with $G/N$.
    }
\end{thm}

\begin{proof}
    $G/N$ is abelian by \Bcr{grad:st:1}. Recall the symbols: 
    \begin{EqLN}
        \defsubgrdcl    
    \end{EqLN}
    
   Consider the sum $\Sum_{k \in G/N} \Der_k$.

   \begin{itemize}
       \item Firstly, $\Sum_{k \in G/N} \Der_k$ is equal to $Der$ due to .
   \end{itemize}
    
\end{proof}
